MoBYv2AL: Self-supervised Active Learning for Image Classification

Active learning(AL) has recently gained popularity for deep learning(DL) models. This is due to efficient and informative sampling, especially when the learner requires large-scale labelled datasets. Commonly, the sampling and training happen in stages while more batches are added. One main bottleneck in this strategy is the narrow representation learned by the model that affects the overall AL selection. We present MoBYv2AL, a novel self-supervised active learning framework for image classification. Our contribution lies in lifting MoBY, one of the most successful self-supervised learning algorithms, to the AL pipeline. Thus, we add the downstream task-aware objective function and optimize it jointly with contrastive loss. Further, we derive a data-distribution selection function from labelling the new examples. Finally, we test and study our pipeline robustness and performance for image classification tasks. We successfully achieved state-of-the-art results when compared to recent AL methods. Code available: https://github.com/razvancaramalau/MoBYv2AL

==> parts/conc.tex <==
We have presented an SSL-based  AL framework for image classification. The main contributions lie in the task-aware contrastive learning pipeline. MoBYv2 retains the higher visual concepts and aligns them with the downstream task. The end-to-end training is efficient and modular, allowing diverse learners and sampling functions. We conduct quantitative experiments and demonstrate the state-of-the-art on four datasets. Our method shows robustness even in simulated class-imbalanced data pools. 

==> parts/intro.tex <==
% \section{Introduction}
\label{sec:intro}
Active learning ~\cite{Sinha2019VariationalLearning,ugcn,Yoo2019LearningLearning,KimConfidentAnalysis, cdal,csal, bengar2021reducing,kim2021task} has gained more popularity in the research community in recent times. The goal of AL is to sample the most \emph{informative} and \emph{diverse} examples from a large pool of unlabelled data to query their labels. Based on the selection criteria, the existing AL methods can be grouped into two. The first group is
uncertainty-based algorithms~\cite{mcdropoutal,Yoo2019LearningLearning,Gal2016DropoutGhahramani} that select complex and informative examples. Whereas representative-based algorithms select the most diverse examples from the data set. To select diverse examples, existing methods first project the images into a feature space followed by applying sampling techniques such as CoreSet~\cite{Sener2017ActiveApproach}. 
Our work falls in the latter category.  

Prominent works on representative-based methods for AL in the past few years have tackled 
a wide range of architectures to learn the image representations such as Convolutional Neural Network~\cite{Yoo2019LearningLearning}, Graph Convolutional  Neural Networks~\cite{ugcn}, Bayesian Network~\cite{caramalau2021active}, Variational Auto-Encoders~\cite{Sinha2019VariationalLearning,kim2021task}, 
and too few to mention. These works have proven that the learned features of the images have directly 
influenced the performance of the pipeline. However, these methods suffer from \emph{cold-start problem}. As we know, in the early selection stage, there are only limited annotated examples, and the above-mentioned architectures
are hard to train with the small training set. Thus, the features extracted from such models get biased from the beginning and continue to become sub-optimal in the subsequent selection stages. This problem is commonly known as \emph{cold-start problem}. To address such a problem, recent works in AL have explored self-supervised learning methods~\cite{csal, bengar2021reducing, altod, revival_iccv21}. 


Self-supervised learning methods~\cite{mixmatch,xie2021moby,dino,moco,byol} have made tremendous progress to generate discriminative representations of the images. Some of the methods have even come close to supervised methods in generalization~\cite{chen2020mocov2,byol,xie2021moby}. One of the earliest works in this direction~\cite{csal} employed consistency loss between the input image and its geometrically augmented versions along with the objective of downstream tasks. However, this method limits augmentation methods in the primitive form. Similarly, J. Bengar et. al~\cite{bengar2021reducing} introduced contrastive learning in AL, but the self-supervised method and end-task objective are optimised in multi-stage form. This makes the model sub-optimal, and it affects the representativeness of the features during selection. Simple random labelling overpasses any AL criteria. Thus, the existing works in this direction show explicit limitations. 

To address these issues, we introduce a novel component, MoBYv2, in our AL pipeline. This component optimises the loss of both the downstream task and self-supervised loss jointly, as shown in Figure~\ref{fig:pipeline}. 
The self-supervised loss is inspired from MoBY~\cite{xie2021moby}, which inherits the strength of 
two popular SSL methods: MoCo~\cite{moco} and BYOL~\cite{byol}. We choose the MoBY~\cite{xie2021moby}  because it addresses the computational complexities and shortcomings of other previous methods such as SimCLR~\cite{simclr} or BYOL\cite{byol}. MoBY
has two branches (as shown in Figure~\ref{fig:pipeline}), one updates with gradient (query encoder) and 
another with momentum (key encoder). The parameters of the momentum encoder are updated in slow-moving average with query one. Moreover, the memory bank of keys from the momentum encoder keeps long dependencies with several mini-batches. Apart from minimising a contrastive loss, another advantage consists in the asymmetric structure of BYOL that captures distances from mean representation. MoBYv2 culminates the AL process of selection with the concept-aware function, CoreSet.

We state our contributions and achievements through: a task-aware self-supervised method jointly trained with the learner; 
a quantitative evaluation on multiple image classification benchmarks such as: CIFAR-10/100\cite{cifar}, SVHN\cite{Goodfellow2014svhn} and FashionMNIST \cite{Xiao2017Fashion-MNIST:Algorithms};
state-of-the-art performance over the existing AL baselines.
% \begin{itemize}

% \end{itemize}

% -----------------------------------------------------------------------------------------------------------------
 
% and the methods to select the diverse examples~\cite{}. The performance of both these categories of methods relies on the feature representations of the images~\cite{}. Thus several architectures such as employed to induce critical features for selection. Recently, self-supervised learning methods such as~\cite{bengar2021reducing, } are explored to induce rich representations for selecting the examples.  The drawback of this method is that pipeline is trained in multi-stage manner. 

 
% Some of the important self-supervised learning method explored so far in active learning are: SimCLR, .. .etc. 
% SimCL needs large-batch size, not scalable. Moreover, 

% MoBY does implicit normalization which makes it memory efficient. And queuing of negative examples in MOBY V2 gives xxxx advantage which is suitable for active learning.


% \textit{While encoder is updated by back-propagation as in SimCLR, momentum encoder is updated by linear interpolation of the two encoders. , the parameters of momentum encoder are updated in consistency with encoder. As a consequence, the keys generated from momentum encoder with different mini-batches are also consistent. }






% \begin{enumerate}
%     \item Active learning is an iterative/online process to select diverse and discriminative examples.
%     \item Existing methods do not exploit unlabelled data to induce representation for sampling.
%     \item Recently, self-supervised methods such as contrastive learning are being effective~\cite{}. \textcolor{red}{What is the drawback of these architectures?}
%     \item  Since AL is an iterative and online process, gives us long-range dependency between labelled and unlabelled examples, importance of exponential gradients update, 
%     \item 
% \end{enumerate}

